Know Unreported Roadway Incidents in Real-time: Early Traffic Anomaly Detection

This research aims to know traffic anomalies as early as possible. A traffic anomaly refers to a generic incident on the road that influences traffic flow and calls for urgent traffic management measures. `Knowing'' the occurrence of a traffic anomaly is twofold: the ability to detect this anomaly before it is reported anywhere, or it may be such that an anomaly can be predicted before it actually occurs on the road (e.g., non-recurrent traffic breakdown). In either way, the objective is to inform traffic operators of unreported incidents in real time and as early as possible. The key is to stay ahead of the curve. Time is of the essence. Conventional automatic incident detection (AID) methods often struggle with early detection due to their limited consideration of spatial effects and early-stage characteristics. Therefore, we propose a deep learning framework utilizing prior domain knowledge and model-designing strategies. This allows the model to detect a broader range of anomalies, not only incidents that significantly influence traffic flow but also early characteristics of incidents along with historically unreported anomalies. We specially design the model to target the early-stage detection/prediction of an incident. Additionally, unlike most conventional AID studies, our method is highly scalable and generalizable, as it is fully automated with no manual selection of historical reports required, relies solely on widely available low-cost data, and requires no additional detectors. The experimental results across numerous road segments on different maps demonstrate that our model leads to more effective and early anomaly detection.

==> tables/blue_table.tex <==
\begin{table}[!htb]
\fontsize{10}{7.2}\selectfont
\begin{center}
{\arrayrulecolor{blue}  % 修改表格线颜色
\color{blue}            % 修改文字颜色
\begin{tabular}{c|c|c|c|c|c|c}
    \hline 
    \multirow{2}*{$\theta_{\text{SD}}^{\text{I-70E}}$ (mph)}
    & \multirow{2}*{Ahead-Labeling} 
    & \multirow{2}*{DR}
    & \multirow{2}*{MTTD} 
    & \multirow{2}*{FAR} 
    & \multirow{2}*{DR(S)} 
    & \multirow{2}*{MTTD(S)}\\
    & &  & & &  & \\\hline
    \multirow{2}*{30} & \multirow{2}*{\xmark} & \multirow{2}*{0.46} & \multirow{2}*{-7} & \multirow{2}*{0.00} & \multirow{2}*{1.00} & \multirow{2}*{-7} \\
    & & & & & & \\
    \multirow{2}*{30} & \multirow{2}*{\cmark} & \multirow{2}*{0.46} & \multirow{2}*{-12} & \multirow{2}*{0.23} & \multirow{2}*{1.00} & \multirow{2}*{-12} \\
    & & & & & & \\
    \multirow{2}*{25} & \multirow{2}*{\xmark} & \multirow{2}*{0.61} & \multirow{2}*{-7} & \multirow{2}*{0.15} & \multirow{2}*{1.00} & \multirow{2}*{-7} \\
    & & & & & & \\
    \multirow{2}*{25} & \multirow{2}*{\cmark} & \multirow{2}*{0.61} & \multirow{2}*{-9} & \multirow{2}*{0.20} & \multirow{2}*{1.00} & \multirow{2}*{-9} \\
    & & & & & & \\
    \multirow{2}*{20} & \multirow{2}*{\xmark} & \multirow{2}*{0.46} & \multirow{2}*{-6} & \multirow{2}*{0.11} & \multirow{2}*{0.75} & \multirow{2}*{-6} \\
    & & & & & & \\
    \multirow{2}*{20} & \multirow{2}*{\cmark} & \multirow{2}*{0.92} & \multirow{2}*{-17} & \multirow{2}*{0.34} & \multirow{2}*{1.00} & \multirow{2}*{-24} \\
    & & & & & & \\
    \hline
\end{tabular}
}
\end{center}
\caption{\textcolor{blue}{Sensitivity Analysis}}\label{tab:sen}
\end{table}

==> tables/bluecopy.tex <==
\begin{algorithm}
\caption*{\textcolor{blue}{Algorithm 3: Threshold Adaptation}}  % 显示编号但不计入自动编号
\begin{footnotesize}
\begin{algorithmic}
\State \textcolor{blue}{\underline{\textbf{Inputs}}:} 
\parbox[t]{\dimexpr\linewidth-\algorithmicindent}{
\textcolor{blue}{Training set $\mathcal{D}_{\text{train}}$,} \\
\textcolor{blue}{Threshold tuning set $\mathcal{D}_{\text{tune}}$,} \\
\textcolor{blue}{Validation set $\mathcal{D}_{\text{val}}$,} \\
\textcolor{blue}{Number of epochs $E$}
}

\State \textcolor{blue}{\underline{\textbf{Outputs}}:}
\textcolor{blue}{Best model parameters $\theta^*$, optimal threshold $\tau^*$}

\State \textcolor{blue}{initialize model parameters $\theta$}
\State \textcolor{blue}{initialize best validation F1 score F$1_{best} \gets 0$}
\For{\textcolor{blue}{$epoch = 1$ to $E$}}
    \State \textcolor{blue}{Train the model $\theta$ on $\mathcal{D}_{\text{train}}$ using WBCE loss}
    \State \textcolor{blue}{initialize best threshold F1 score F$1_{\tau} \gets 0$}
    \For{\textcolor{blue}{$\tau = 0.01, 0.02, \ldots, 0.99$}}
        \State \textcolor{blue}{Apply model $\theta$ to $\mathcal{D}_{\text{tune}}$ with threshold $\tau$}
        \State \textcolor{blue}{Compute F1 score $\text{F}1_{\tau'}$ under threshold $\tau$}
        \If{\textcolor{blue}{F$1_{\tau'} > \text{F}1_{\tau}$}}
            \State \textcolor{blue}{$\text{F}1_{\tau} \gets \text{F}1_{\tau'}$}
            \State \textcolor{blue}{$\tau^* \gets \tau$}
        \EndIf
    \EndFor
    \State \textcolor{blue}{Apply model $\theta$ to $\mathcal{D}_{\text{val}}$ using threshold $\tau^*$}
    \State \textcolor{blue}{Compute validation F1 score $\text{F}1_{val}$}
    \If{\textcolor{blue}{$\text{F}1_{val} > \text{F}1_{best}$}}
        \State \textcolor{blue}{$\text{F}1_{best} \gets \text{F}1_{val}$}
        \State \textcolor{blue}{Save model parameters $\theta^* \gets \theta$}
    \EndIf
\EndFor

\end{algorithmic}
\end{footnotesize}
\end{algorithm}
